An Interpretable Rule Creation Method for Black-Box Models based on Surrogate Trees -- SRules

As artificial intelligence (AI) systems become increasingly integrated into critical decision-making processes, the need for transparent and interpretable models has become paramount. In this article we present a new ruleset creation method based on surrogate decision trees (SRules), designed to improve the interpretability of black-box machine learning models. SRules balances the accuracy, coverage, and interpretability of machine learning models by recursively creating surrogate interpretable decision tree models that approximate the decision boundaries of a complex model. We propose a systematic framework for generating concise and meaningful rules from these surrogate models, allowing stakeholders to understand and trust the AI system's decision-making process. Our approach not only provides interpretable rules, but also quantifies the confidence and coverage of these rules. The proposed model allows to adjust its parameters to counteract the lack of interpretability by precision and coverage by allowing a near perfect fit and high interpretability of some parts of the model . The results show that SRules improves on other state-of-the-art techniques and introduces the possibility of creating highly interpretable specific rules for specific sub-parts of the model.

==> sections/10_Annexes.tex <==
\appendix
\section{Annexes}


\subsection{Results}


\begin{table}
 \centering
 \caption{Ensemble Non Recursive F1-score}

\resizebox{\columnwidth}{!}{%
 \begin{tabular}{c||c||c||c|c|cc|cc|cc}
 \hline
\textbf{Method}& \textbf{Dataset}  & \textbf{Coverage} & \textbf{DT} & \textbf{Ensemble} & \textbf{RFIT} & \textbf{RFIT \# rl. num.} & \textbf{RC} & \textbf{RC \# rl. num.} & \textbf{SR} & \textbf{SR \# rl. num.} \\ \hline 
 RF & divorce & 90.78±14.22 & 87.4±29.47 & 88.55±29.63 & 87.9±29.49 & 25.73±3.64 & 87.55±29.53 & 5.63±0.55 & 86.5±29.37 & 2.83±0.69 \\ 
 RF & kr-vs-kp & 75.12±5.54 & 98.04±1.5 & 99.84±0.22 & 98.86±0.97 & 21.9±2.86 & 94.25±1.62 & 4.1±0.3 & 98.91±1.03 & 10.8±1.356 \\ 
 RF & wisconsin & 71.04±12.58 & 98.44±1.73 & 98.83±1.28 & 99.03±1.51 & 19.1±2.13 & 98.69±1.49 & 8.47±1.38 & 98.49±1.77 & 5.03±1.82 \\ 
 RF & SPECT & 40.37±5.78 & 93.5±3.19 & 93.5±3.19 & 94.76±4.31 & 22.88±1.69 & 93.5±3.19 & 5.0±1.0 & 93.5±3.19 & 1.0±0.0 \\
 RF & salud-covid & 52.88±9.68 & 70.19±13.28 & 76.73±9.72 & 71.55±15.56 & 18.93±1.75 & 58.07±24.15 & 6.43±1.26 & 77.88±9.98 & 11.6±2.27\\
 RF & tic-tac-toe & 45.31±8.14 & 97.04±3.48 & 99.73±0.6 & 97.92±3.11 & 21.03±1.87 & 87.8±4.93 & 3.6±0.55 & 98.93±1.4 & 22.67±3.75\\ \hline
 RF & Total Average & 62.58±9.32 &	90.77±8.78 &	92.86±7.44 &	91.67±9.16 &	21.60±2.32 &	86.64±10.82 &	5.54±0.84 &	92.37±7.79 &	8.99±1.65\\ \hline


 GBC & divorce & 90.78±14.22 & 87.4±29.47 & 88.55±29.63 & 87.9±29.49 & 25.73±3.64 & 87.55±29.53 & 5.63±0.55 & 86.5±29.37 & 2.83±0.69 \\ 
 GBC & kr-vs-kp & 75.83±5.75 & 98.0±1.64 & 99.77±0.28 & 98.91±0.9 & 21.8±3.21 & 94.33±1.58 & 4.23±0.42 & 98.96±0.81 & 11.03±1.43 \\ 
 GBC & wisconsin & 71.04±12.58 & 98.44±1.73 & 98.83±1.28 & 99.03±1.51 & 19.1±2.13 & 98.69±1.49 & 8.47±1.38 & 98.49±1.77 & 5.03±1.82 \\ 
 GBC & SPECT & 42.57±14.73 & 93.41±5.29 & 94.82±3.88 & 95.59±3.99 & 21.67±2.87 & 94.82±3.88 & 4.75±0.6 & 94.82±3.88 & 1.25±0.43 \\
 GBC & salud-covid & 52.88±9.68 & 70.19±13.28 & 76.73±9.72 & 71.55±15.56 & 18.93±1.75 & 58.07±24.15 & 6.43±1.26 & 77.88±9.98 & 11.6±2.27 \\
 GBC & tic-tac-toe & 45.31±8.14 & 97.04±3.48 & 99.73±0.6 & 97.92±3.11 & 21.03±1.87 & 87.8±4.93 & 3.6±0.55 & 98.93±1.4 & 22.67±3.75\\\hline
 GBC & Total Average & 63.07±10.85	&90.75±9.15	&93.07±7.57	&91.82±9.09&	21.38±2.58	&86.88±10.93	&5.52±0.79	&92.60±7.87&	9.07±1.73\\ \hline

 ADA & divorce & 94.31±6.35 & 96.84±4.56 & 97.48±4.11 & 98.13±3.21 & 25.77±4.1 & 96.3±5.18 & 5.7±0.59 & 96.92±4.41 & 3.07±0.685 \\ 
 ADA & kr-vs-kp & 57.91±12.51 & 94.82±2.09 & 97.78±0.89 & 97.31±1.68 & 21.97±3.03 & 90.77±2.64 & 4.17±0.37 & 98.63±0.85 & 69.4±10.14 \\ 
 ADA & wisconsin & 75.38±10.07 & 98.02±1.41 & 98.74±1.14 & 98.83±1.09 & 18.83±2.16 & 98.38±1.33 & 8.3±1.51 & 97.74±1.15 & 8.47±2.11 \\ 
 ADA & SPECT & 29.63±0.0 & 85.71±0.0 & 85.71±0.0 & 85.71±0.0 & 22.0±0.0 & 85.71±0.0 & 6.0±0.0 & 85.71±0.0 & 1.0±0.0 \\
 ADA & salud-covid & 38.77±8.26 & 39.66±31.56 & 40.83±34.75 & 36.55±34.05 & 18.67±1.78 & 28.97±33.52 & 6.47±0.96 & 23.73±33.76 & 10.2±2.95 \\
 ADA & tic-tac-toe & 53.16±8.58 & 95.3±5.42 & 99.54±0.89 & 97.39±2.77 & 22.0±2.24 & 86.43±5.14 & 3.67±0.6 & 98.87±1.53 & 20.37±2.54 \\ \hline 
 ADA & Total Average & 58.19±7.63 & 85.06±7.51 & 86.68±6.96 & 85.65±7.13 & 21.54±2.22 & 81.09±7.97 & 5.72±0.67 & 83.60±6.95 & 18.75±3.07\\ \hline


 CAT & divorce & 92.16±11.7 & 94.16±18.0 & 63.38±12.39 & 95.13±17.96 & 24.17±3.26 & 93.96±17.96 & 5.7±0.59 & 95.06±17.91 & 3.07±0.63 \\ 
 CAT & kr-vs-kp & 49.95±9.56 & 99.28±1.66 & 59.54±6.8 & 99.27±1.66 & 21.23±3.57 & 91.3±4.12 & 4.07±0.25 & 99.28±1.66 & 3.2±0.65 \\ 
 CAT & wisconsin & 84.96±4.34 & 98.34±1.09 & 82.36±2.26 & 99.1±0.94 & 19.57±3.06 & 98.39±1.61 & 8.27±1.65 & 98.98±0.85 & 8.6±1.45 \\ 
 CAT & SPECT & 39.96±14.42 & 95.31±4.52 & 95.9±3.97 & 96.0±3.86 & 21.72±2.33 & 95.51±3.83 & 5.38±0.96 & 95.9±3.97 & 2.97±1.1 \\
 CAT & salud-covid & 43.88±9.94 & 74.74±19.07 & 14.33±4.66 & 86.53±14.54 & 18.33±1.89 & 76.81±22.13 & 6.17±0.73 & 87.76±12.66 & 7.4±1.84 \\
 CAT & tic-tac-toe & 49.03±6.29 & 99.48±0.88 & 88.16±3.02 & 100.0±0.0 & 21.33±1.64 & 95.79±4.46 & 3.53±0.56 & 99.66±0.85 & 11.17±2.6 \\ \hline
 CAT & Total Average & 59.99±9.375& 93.55±7.53& 67.27±5.51 & 96.00±6.49 & 21.05±2.625 & 91.96±9.02 & 5.52±0.79 & 96.10±6.31 & 5.20±1.18\\ \hline \hline

 
    \textbf{Global} & \textbf{Total Average} & \textbf{60.96±9.29} & \textbf{90.03±8.24} & \textbf{84.97±6.87} & \textbf{91.29±7.97} & \textbf{21.39±2.44} & \textbf{86.64±9.69} & \textbf{5.58±0.77} & \textbf{91.17±7.23} & \textbf{10.50±1.85} \\ \hline \hline
 \end{tabular}
 } 
 \label{table:results_table_non_recursive}
\end{table}

\begin{table}
 \centering
 \caption{Ensemble Recursive F1-score}

\resizebox{\columnwidth}{!}{%
 \begin{tabular}{c||c||c||c|c|cc|cc|cc}
 \hline

\textbf{Method}& \textbf{Dataset}  & \textbf{Coverage} & \textbf{DT} & \textbf{Ensemble} & \textbf{RFIT} & \textbf{RFIT \# rl. num.} & \textbf{RC} & \textbf{RC \# rl. num.} & \textbf{SR} & \textbf{SR \# rl. num.} \\ \hline
 RF & divorce & 91.96±14.68 & 88.94±24.74 & 51.56±44.22 & 88.54±29.63 & 26.47±3.95 & 87.1±29.33 & 5.67±0.54 & 86.17±29.19 & 3.0±1.34 \\ 
 RF & kr-vs-kp & 92.07±6.47 & 96.19±1.36 & 45.32±20.09 & 97.89±1.27 & 21.57±2.53 & 92.42±1.91 & 4.13±0.34 & 98.5±1.48 & 20.3±3.94 \\ 
 RF & wisconsin & 81.79±11.25 & 97.12±2.01 & 86.72±17.84 & 98.26±1.48 & 19.13±2.9 & 97.85±1.62 & 8.43±2.14 & 97.34±2.03 & 7.33±2.01 \\ 
 RF & SPECT & 50.62±5.52 & 89.83±2.12 & 89.15±9.57 & 89.83±2.12 & 21.5±2.5 & 89.83±2.12 & 5.67±1.7 & 90.62±3.06 & 1.0±0.0 \\
 RF & salud-covid & 60.13±5.56 & 64.2±19.59 & 40.54±15.13 & 69.35±16.39 & 18.5±1.89 & 56.22±19.84 & 6.07±1.18 & 74.54±13.28 & 15.3±3.08\\
 RF & tic-tac-toe & 68.65±10.02 & 95.91±3.83 & 76.16±10.5 & 97.38±2.21 & 21.13±2.01 & 85.94±4.49 & 3.6±0.49 & 98.35±1.93 & 33.23±5.55\\ \hline
 RF & Total Average & 74.20±8.92 & 88.70±8.94 & 64.91±19.56 & 90.21±8.85 & 21.38±2.63 & 84.89±9.89 & 5.60±1.07 & 90.92±8.50 & 13.36±2.65\\ \hline 


 GBC & divorce & 91.96±14.68 & 88.94±24.74 & 51.56±44.22 & 88.54±29.63 & 26.47±3.95 & 87.1±29.33 & 5.67±0.54 & 86.17±29.19 & 3.0±1.34 \\ 
 GBC & kr-vs-kp & 93.5±4.7 & 95.87±1.36 & 52.46±17.44 & 98.0±1.16 & 22.53±3.83 & 91.91±1.94 & 4.07±0.25 & 98.6±1.08 & 18.33±2.66 \\ 
 GBC & wisconsin & 81.79±11.25 & 97.12±2.01 & 86.72±17.84 & 98.26±1.48 & 19.13±2.9 & 97.85±1.62 & 8.43±2.14 & 97.34±2.03 & 7.33±2.01 \\ 
 GBC & SPECT & 50.62±5.52 & 89.83±2.12 & 89.15±9.57 & 89.83±2.12 & 21.5±2.5 & 89.83±2.12 & 5.67±1.7 & 90.62±3.06 & 1.0±0.0 \\
 GBC & salud-covid & 60.13±5.56 & 64.2±19.59 & 40.54±15.13 & 69.35±16.39 & 18.5±1.89 & 56.22±19.84 & 6.07±1.18 & 74.54±13.28 & 15.3±3.08\\
 GBC & tic-tac-toe & 68.65±10.02 & 95.91±3.83 & 76.16±10.5 & 97.38±2.21 & 21.13±2.01 & 85.94±4.49 & 3.6±0.49 & 98.35±1.93 & 33.23±5.55\\ \hline
 GBC & Total Average & 74.44±8.62 &	88.65±8.94 &	66.10±19.12 &	90.23±8.83 &	21.54±2.85 &	84.81±9.89 &	5.59±1.05 &	90.94±8.43 &	13.03±2.44\\ \hline



 ADA &	divorce & 93.14±9.74 & 92.61±17.75 & 65.76±38.3 & 94.45±17.83 & 24.97±2.27 & 92.48±17.79 & 5.7±0.59 & 91.89±17.82 & 3.8±1.8 \\ 
 ADA &	kr-vs-kp & 83.45±5.82 & 95.53±1.06 & 80.55±12.44 & 97.33±1.26 & 21.73±3.13 & 91.92±1.86 & 4.1±0.3 & 95.85±3.44 & 106.3±14.45 \\ 
 ADA &	wisconsin & 81.24±7.57 & 97.57±2.11 & 87.99±14.52 & 98.61±1.15 & 19.37±2.21 & 98.3±1.38 & 8.63±1.91 & 97.13±2.29 & 8.83±2.1 \\ 
 ADA &	SPECT & 28.28±14.42 & 92.38±8.13 & 88.83±19.55 & 91.19±18.48 & 22.18±1.93 & 93.91±6.69 & 5.29±1.1 & 94.1±6.93 & 3.61±1.29 \\
 ADA &	salud-covid & 52.28±7.1 & 52.32±22.95 & 46.69±19.69 & 53.33±23.21 & 18.03±1.64 & 33.77±25.26 & 6.27±1.0 & 43.2±31.03 & 21.33±7.03 \\
 ADA &	tic-tac-toe & 72.2±7.49 & 95.14±4.28 & 86.57±4.9 & 97.31±2.01 & 22.13±2.31 & 84.3±4.59 & 3.7±0.74 & 99.23±0.97 & 31.0±4.43 \\ \hline
 ADA &	Total Average & 68.43±8.69 &	87.59±9.38 &	76.07±18.23 &	88.70±10.66 &	21.40±2.25 &	82.45±9.60 &	5.62±0.94 &	86.90±10.41 &	29.15±5.18\\ \hline


 CAT & divorce & 93.92±6.35 & 98.49±2.76 & 65.75±3.49 & 98.66±3.14 & 25.5±3.37 & 97.03±4.86 & 5.73±0.57 & 98.06±2.98 & 3.73±1.77 \\ 
 CAT & kr-vs-kp & 89.99±4.03 & 96.88±1.83 & 69.76±2.66 & 98.43±1.08 & 21.47±3.06 & 93.05±2.42 & 4.13±0.34 & 98.76±1.11 & 16.23±3.5 \\ 
 CAT & wisconsin & 87.07±5.25 & 98.04±1.63 & 81.77±2.25 & 99.17±1.2 & 18.93±1.77 & 98.38±1.72 & 8.0±1.53 & 98.64±1.52 & 9.2±1.17 \\ 
 CAT & SPECT & 45.0±15.13 & 94.69±5.37 & 95.81±4.68 & 95.99±4.74 & 21.85±2.63 & 95.68±4.71 & 5.44±1.37 & 95.81±4.68 & 2.7±1.41 \\
 CAT & salud-covid & 58.28±6.1 & 64.37±20.78 & 15.29±4.05 & 71.47±14.13 & 18.5±1.96 & 58.35±21.51 & 6.4±1.08 & 73.47±15.63 & 12.0±2.83\\
 CAT & tic-tac-toe & 62.77±6.25 & 97.54±1.66 & 84.68±3.42 & 98.26±1.76 & 21.4±1.85 & 91.38±4.3 & 3.8±0.54 & 98.64±1.26 & 21.43±4.35 \\ \hline 
 CAT & Total Average & 72.84±7.19 & 91.67±5.67 & 68.84±3.43 & 93.66±4.34 & 21.28±2.44 & 88.98±6.59 & 5.58±0.91 & 93.90±4.53 & 10.88±2.51\\ \hline \hline

     \textbf{Global}& \textbf{Total Average} & \textbf{72.48±8.36} & \textbf{89.15±8.23} & \textbf{68.98±15.09} & \textbf{90.70±8.17} & \textbf{21.40±2.54} & \textbf{85.28±8.99} & \textbf{5.60±0.99} & \textbf{90.67±7.97} & \textbf{16.61±3.15}\\ \hline \hline

 \end{tabular}
 } 
 \label{table:results_table_recursive}
\end{table}


